Is a Peeled Apple Still Red? Evaluating LLMs' Ability for Conceptual Combination with Property Type

Conceptual combination is a cognitive process that merges basic concepts, enabling the creation of complex expressions. During this process, the properties of combination (e.g., the whiteness of a peeled apple) can be inherited from basic concepts, newly emerge, or be canceled. However, previous studies have evaluated a limited set of properties and have not examined the generative process. To address this gap, we introduce the Conceptual Combination with Property Type dataset (CCPT), which consists of 12.3K annotated triplets of noun phrases, properties, and property types. Using CCPT, we establish three types of tasks to evaluate LLMs for conceptual combination thoroughly. Our key findings are threefold: (1) Our automatic metric grading property emergence and cancellation closely corresponds with human judgments. (2) LLMs, including OpenAI's o1, struggle to generate noun phrases which possess given emergent properties. (3) Our proposed method, inspired by cognitive psychology model that explains how relationships between concepts are formed, improves performances in all generative tasks. The dataset and experimental code are available at https://github.com/seokwon99/CCPT.git.

==> Tables/llama_ft.tex <==
\begin{table*}[ht!]
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccccccc}
\Xhline{1.2pt} 
&\multicolumn{6}{c}{\textbf{\textsc{Property Induction}}}&\multicolumn{3}{c}{\textbf{\textsc{Noun Phrase Completion}}}\\\cline{2-10}
&\multicolumn{3}{c}{\textbf{(1) \textsc{Emergent}}}&\multicolumn{3}{c}{\textbf{(2) \textsc{Canceled}}}&\multicolumn{3}{c}{\textbf{(3) \textsc{Emergent}}}\\\cline{2-10}
&$R_{\mathcal{H},\mathcal{M},\mathcal{P}}$\downarrow&$R_{\mathcal{N},\mathcal{P}}$\uparrow&$\mathcal{E}$\uparrow&$R_{\mathcal{H},\mathcal{M},\mathcal{P}}$\uparrow&$R_{\mathcal{N},\mathcal{P}}$\downarrow&$\mathcal{C}$\uparrow&$R_{\mathcal{H},\mathcal{M},\mathcal{P}}$\downarrow&$R_{\mathcal{N},\mathcal{P}}$\uparrow&$\mathcal{E}$\uparrow\\\hline
\textbf{\textit{LLaMa-3.1-8B}}&40 $\pm$ 1.3&66 $\pm$ 0.3&33 $\pm$ 0.6&&&&48 $\pm$ 2.5&57 $\pm$ 1.9&18 $\pm$ 1.2 \\
+ QLoRA (NF4, r=16)&41 $\pm$ 0.8&63 $\pm$ 1.7&32 $\pm$ 1.7&&&&57 $\pm$ 2.5&69 $\pm$ 2.7&19 $\pm$ 1.9 \\
+ Full&&&&&&&&& \\\midrule
\textbf{\textit{LLaMa-3.1-70B}}&41 $\pm$ 0.5&81 $\pm$ 0.8&43 $\pm$ 1.1&&&&49 $\pm$ 1.7&68 $\pm$ 1.0&23 $\pm$ 1.2 \\
+ QLoRA (NF4, r=16)&40 $\pm$ 0.5&82 $\pm$ 0.5&45 $\pm$ 0.6&&&&39 $\pm$ 0.2 &66 $\pm$ 1.4&32 $\pm$ 0.5 \\\midrule
\textbf{\textit{Gold}}&25&92&67&92&6&86&25&92&67 \\\Xhline{1.2pt} 
\end{tabular}
}
\caption{Generative results of LLaMA-3.1~\cite{dubey2024llama} baseline models across two sizes are presented for property induction and noun phrase completion tasks. For the full-parameter setting, models are fine-tuned using fp32 precision scaling.}
\label{table:llama_ft}
\vspace{-5mm}
\end{table*}

==> Tables/property_type_prediction_multiple_models.tex <==
\begin{table}[!t]
    \centering
    \small
    \renewcommand{\arraystretch}{1.5}
    \setlength{\aboverulesep}{0pt}
    \setlength{\belowrulesep}{0pt}
    \resizebox{\linewidth}{!}{
\begin{tabular}{lcc}
\hline
& Accuracy & F1 \\hline
\textit{\textbf{LLaMa-70B}} & & \\\hline
\textit{\textbf{QWEN-72B}} & & \\
\textit{\textbf{GPT-4o}} & & \\
\textit{\textbf{o1-mini}} & & \\
\textit{\textbf{o1-preview}} & & \\\hline
\hline
\end{tabular}}
    \caption{Classification results of property type prediction on 400 sampled instances, 100 samples for each property type. We report the accuracy and a macro-averaged F1 score.}
    \label{tab:type_prediction_multi_models}
\end{table}

==> Tables/result_cls.tex <==
\begin{table}[t!]
\centering
\renewcommand{\arraystretch}{1.4}
% \setlength\tabcolsep{2.5pt}
\footnotesize
% \begin{tabular}{ll}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lcccc}
\midrule
\multicolumn{1}{c}{}            & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Property\\ Induction\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Noun Phrase\\ Completion\end{tabular}} \\ \toprule
                                & E                                   & C                                          & E                                     & C                                            \\ \midrule
\textbf{Random}                 & 25                                  & 25                                         & 25                                    & 25                                           \\ \midrule
\textit{\textbf{LLaMa}} &                                     &                                            &                                       &                                              \\
Naive                       &                                     &                                            &                                       &                                              \\
CoT                         &                                     &                                            &                                       & \textbf{}                                    \\
RAG                           &                                     & \textbf{}                                  &                                       & \textbf{}                                    \\\midrule
\textit{\textbf{Qwen}} &                                     &                                            &                                       &                                              \\
Naive                       &                                     &                                            &                                       &                                              \\
CoT                         &                                     &                                            &                                       & \textbf{}                                    \\
RAG                           &                                     & \textbf{}                                  &                                       & \textbf{}                                    \\\midrule
\textit{\textbf{GPT-4o}}        &                                     &                                            &                                       &                                              \\
Naive                       & 70                                  & 62                                         & 66                                    & 52                                           \\
CoT                         & 72                                  & 66                                         & 64                                    & 52                                           \\
RAG                           & 68                                  & 62                                         & 62                                    & 56                                           \\\midrule
\textbf{Human}                  &                                     &                                            & 89                                    &                                              \\ \bottomrule
\end{tabular}
}
\vspace{-3mm}
\caption{Accuracies (\%) of various LLM baselines with discriminative setting on the two downstream tasks: Noun Phrase Completion and Property Induction . All downstream tasks are 4-way classification problems. E and C denote \textit{emergent property} and \textit{canceled property} setting, respectively.}
\vspace{-3mm}
\label{table:cls_result}
\end{table}

==> Tables/result_gen_human_gpt4oeval.tex <==
\begin{table*}[t!]
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccccccc}
\Xhline{1.2pt} 
&\multicolumn{6}{c}{\textbf{\textsc{Property Induction}}}&\multicolumn{3}{c}{\textbf{\textsc{Noun Phrase Completion}}}\\\cline{2-10}
&\multicolumn{3}{c}{\textbf{(1) \textsc{Emergent}}}&\multicolumn{3}{c}{\textbf{(2) \textsc{Canceled}}}&\multicolumn{3}{c}{\textbf{(3) \textsc{Emergent}}}\\\cline{2-10}
\textbf{\textit{GPT-4o}}&$R_{\mathcal{H},\mathcal{M},\mathcal{P}}$\downarrow&$R_{\mathcal{N},\mathcal{P}}$\uparrow&$\mathcal{E}$\uparrow&$R_{\mathcal{H},\mathcal{M},\mathcal{P}}$\uparrow&$R_{\mathcal{N},\mathcal{P}}$\downarrow&$\mathcal{C}$\uparrow&$R_{\mathcal{H},\mathcal{M},\mathcal{P}}$\downarrow&$R_{\mathcal{N},\mathcal{P}}$\uparrow&$\mathcal{E}$\uparrow\\\hline
Base   & 49.2 & 84.1 & 36.3 & 70.7 & 29.4 & 43.9 & 54.3 & 69.0 & 20.4 \\
CoT     & 45.4 & 84.1 & 41.3 & 68.0 & 21.5 & 47.0 & 53.0 & \textbf{77.8} & \textul{26.7} \\
S.A.w/ LLM & \textbf{43.0} & 84.4 & \textbf{43.3} & \textbf{79.0} & 23.1 & \textbf{57.6} & 52.6 & 69.6 & 22.0 \\
S.A.w/ ConceptNet & \textul{44.8} & \textbf{86.1} & \textul{42.2} & 75.9 & \textbf{19.6} & \textul{56.5} & \textbf{48.7} & 65.4 & 20.2 \\
S.A.w/ Both & 47.4 & \textul{84.6} & 40.2 & \textul{77.8} & 22.8 & 56.1 & \textul{50.9} & \textul{75.9} & \textbf{29.6} \\\hline
\textbf{\textit{Human}}& 42.8 & 84.8 & 44.3 & 73.5 & 22.4 & 52.6 & 43.7 & 79.8 & 39.0 \\\hline
\textbf{\textit{Gold}} & 34.4 & 87.2 & 52.8 & 79.6 & 21.1 & 59.0 & 33.0 & 90.6 & 57.6 \\\Xhline{1.2pt} 
\end{tabular}
}
\caption{GPT-4o evaluation of generative results on sub-sampled test instances in Table~\ref{table:gen_result_human}. \textbf{Bold numbers} indicate the best scores, while \underline{underline} numbers are the second-best.}
\label{table:gen_result_human_gpt4o_eval}
\vspace{-5mm}
\end{table*}
